Runtime Concurrency Control and Operation Scheduling for High Performance Neural Network Training

Training neural network often uses a machine learning framework such as TensorFlow and Caffe2. These frameworks employ a dataflow model where the NN training is modeled as a directed graph composed of a set of nodes. Operations in neural network training are typically implemented by the frameworks as primitives and represented as nodes in the dataflow graph. Training NN models in a dataflow-based machine learning framework involves a large number of fine-grained operations. Those operations have diverse memory access patterns and computation intensity. How to manage and schedule those operations is challenging, because we have to decide the number of threads to run each operation (concurrency control) and schedule those operations for good hardware utilization and system throughput. In this paper, we extend an existing runtime system (the TensorFlow runtime) to enable automatic concurrency control and scheduling of operations. We explore performance modeling to predict the performance of operations with various thread-level parallelism. Our performance model is highly accurate and lightweight. Leveraging the performance model, our runtime system employs a set of scheduling strategies that co-run operations to improve hardware utilization and system throughput. Our runtime system demonstrates a big performance benefit. Comparing with using the recommended configurations for concurrency control and operation scheduling in TensorFlow, our approach achieves 33% performance (execution time) improvement on average (up to 49%) for three neural network models, and achieves high performance closing to the optimal one manually obtained by the user.

==> text/op_characterizations.tex <==
\section{Operation Characterization (2-3P)}
\label{sec:op}
We study and characterize performance of operations in 
xxx neural network models. We use the operation characterization to drive the design of our runtime to optimize concurrency and NUMA data locality. 

Unless indicated otherwise, we use a machine with two Intel Xeon E5-2630 v3 CPUs (8 cores each CPU and 16 cores in total) for our performance study. The CPU supports hyper-threading, so we can run 32 threads at most. Given such architecture, we have two NUMA nodes in the machine.  

\subsection{Timeline and Statistics Analysis}

Figures~\ref{fig:models-time}~\ref{fig:models-invocation}~\ref{fig:models-queue} illustrate operations' timeline and statistics of training the three CNN models. Operations' timeline and statistics are generated by TensorBoard and processed by Python based scripts. From these three figures, we can make following significant observations.

\textbf{Observation 1:} Each training step includes a few large operations and many small operations. Figure~\ref{fig:models-time} illustrates the execution time of each operation to the total execution time of three CNNs separately and sorts operations in terms of decreased execution time. The execution time of top 10 operations account for 85\% in DCGAN, 85\% in Inception and 90\% in ResNet. However, in Figure~\ref{fig:models-invocation}, invocation times of these top 10 operations are only 23\% in DCGAN, 34\% in Inception and 38\% in ResNet. 

\textbf{Observation 2:} There are adequate operations ready to launch in parallel. Figure~\ref{fig:models-queue} shows the number of operations in a waiting queue, a queue which includes operations executed without dependencies, when an operation is either put into the queue for waiting or is left the queue for execution. At the beginning, three CNN models need to initialize variables and the operations in this process barely need dependent operations. Thus, Figure~\ref{fig:models-queue} shows large amount of operations in the waiting queue. For most of the case, the number of operations in the waiting queue is 2-4 in DCGAN, 2-12 in Inception and 2-5 in ResNet. In the runtime scheduling, threads utilization can be improved  by co-running operations in the waiting queue to increase inter-operations parallelism. 

\textbf{Observation 3:} The execution time accumulation of small operations is large. The execution time of each small operation accounts for small percentage compared to large operations, but the execution time accumulation of small operations is also large compared to the total execution time. In the runtime design, we should also consider scheduling small operations to further improve performance.


\begin{figure*}
\begin{subfigure}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in]
{./figures/DCGAN_Timeline.pdf}
\caption{DCGAN}
\label{fig:DCGAN-time}
\end{subfigure}%
\begin{subfigure}[t]{0.34\linewidth}
\centering
\includegraphics[width=2.35in]{./figures/Inception_Timeline.pdf}
\caption{Inception}
\label{fig:Inception-time}
\end{subfigure}%
\begin{subfigure}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.2in]{./figures/ResNet_Timeline.pdf}
\caption{ResNet}
\label{ResNet-time}
\end{subfigure}
\caption{Execution time breakdown of three CNN models} \label{fig:models-time}
\end{figure*}

\begin{figure*}
\begin{subfigure}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.3in]
{./figures/DCGAN_Invocation.pdf}
\caption{DCGAN}
\label{fig:DCGAN-invocation}
\end{subfigure}%
\begin{subfigure}[t]{0.34\linewidth}
\centering
\includegraphics[width=2.3in]{./figures/Inception_Invocation.pdf}
\caption{Inception}
\label{fig:Inception-invocation}
\end{subfigure}%
\begin{subfigure}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.3in]{./figures/ResNet_Invocation.pdf}
\caption{ResNet}
\label{ResNet-invocation}
\end{subfigure}
\caption{Operation invocation times of three CNN models} \label{fig:models-invocation}
\end{figure*}

\begin{figure*}
\begin{subfigure}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.3in]
{./figures/DCGAN_queue.pdf}
\caption{DCGAN}
\label{fig:DCGAN-queue}
\end{subfigure}%
\begin{subfigure}[t]{0.34\linewidth}
\centering
\includegraphics[width=2.3in]{./figures/Inception_queue.pdf}
\caption{Inception}
\label{fig:Inception-queue}
\end{subfigure}%
\begin{subfigure}[t]{0.33\linewidth}
\centering
\includegraphics[width=2.3in]{./figures/ResNet_queue.pdf}
\caption{ResNet}
\label{ResNet-queue}
\end{subfigure}
\caption{The number of operations in a waiting queue without dependencies in three CNN models} \label{fig:models-queue}
\end{figure*}


%\subsection{Roofline Performance Analysis}
\subsection{Operation Concurrency}
The operation-based ML frameworks must decide the number of threads
to run each operation (i.e., intra-op parallelism) and how many operations can co-run (i.e., inter-op parallelism). Intra-op and inter-op parallelisms have great impact on performance. 


\textcolor{blue}{Profiling methodology: }
Challenges: offline profiling needs operation interfaces while some operations don't have such interfaces.

Your solutions.




%\textbf{Roofline model}

\textbf{Best thread number}


%roofline, AIT and bandwidth; \\


\subsection{NUMA Locality}
%\textbf{NUMA background.}
%Modern servers are generally built with more than processor to provide enough computing capacity. Which puts more pressure on data feeding. The CPUs have been starved for data for more than half a century since the 1960s with the advent of the first supercomputer. The NUMA (Non-Uniform Memory Access) architecture attempts to solve this problem by providing separate memory for each processor. NUMA improve the performance for problems involving spread data, like inter paralleled ops in tensorflow. The involvement of NUMA comes with a mismatching of the hardware architecture and applications, just like any upgrading of hardware. Only when the threads and data are congruously placed on a processor and its local memory. While general applications use a uniform memory address space and see the memory as an indivisible whole. This has been a hot researching topic for past decade years.

%To detect the performance influence of the NUMA on tensorflow, we test the performance of tensorflow running on a server equipped two Intel Xeon E5-2630 v3 CPUs (8 cores, Hyper-threading on). Each CPU has 16GB local DRAM. We run inception, resnet and DCGEN on the platform with default configuration of tensorflow (16 inter threads and 16 intra threads). We test Memory latency, Memory Accessing Imbalance and Remote Access Ratio.

We study the performance of tensforflow using its default configuration (i.e., inter-op and intra-op parallelisms are both 16) for
a couple of neural networks. We measure average memory access latency, memory access imbalance across NUMA nodes (i.e., the standard deviation of the load across all NUMA nodes, expressed as percent of the mean), and local access ratio (i.e., the percent of all memory accesses issued from a local node).
%The results are shown in table xxx. Remote access ratio is the percent of all local memory accesses; Memory latency is the average number of cycles to satisfy a memory request from any node; Memory controller imbalance is the standard deviation of the load across all memory controllers, expressed as percent of the mean. Average interconnect (IC) usage shows the utilized interconnect bandwidth as percent of total, averaged across all links, the imbalance shows the standard deviation of utilization across the links as percent of mean utilization.

\begin{table*}[h]\centering
\small
%\renewcommand{\arraystretch}{1.1}
\caption{The Memory Latency and Memory Accessing Imbalance} \label{tab:LatencyAndImbalance}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
 & \multicolumn{3}{|c|}{\textbf{Memory Latency}} & \multicolumn{2}{|c|}{\textbf{Memory Distribution}}\\
 & \multicolumn{3}{|c|}{\textbf{cycles}} & \multicolumn{2}{|c|}{\textbf{Imbalance}}\\
\hline
 &Max&Min&Average&Package 0&Package 1\\
\hline
Conv2DBackpropFilter&828601 &5447 &61546 &88\%&12\%\\
\hline
Conv2DBackpropInput&1164677 &1324 &75161 &86\%&14\%\\
\hline
Mul&1699 &34 &612 &3\%&97\%\\
\hline
Conv2D&2390 &170 &916 &82\%&18\%\\
\hline
Tile&1318 &13 &319 &86\%&14\%\\
\hline
Sub&1146 &10 &253 &0\%&100\%\\
\hline
Sum&337 &5 &40 &89\%&11\%\\
\hline
Mean&883337&19&164128 &100\%&0\%\\
\hline
SquaredDifference&1310 &137 &542 &84\%&16\%\\
\hline
AddN&1395 &1010 &1203 &100\%&0\%\\
\hline
Slice&292596 &13 &5723 &56\%&44\%\\
\hline
MatMult&497 &387 &430 &77\%&23\%\\
\hline
total&1164677 &5 &15255 &83\%&17\%\\
\hline
\end{tabular}%\vspace{-10pt}
\end{table*}

\textbf{Observation 1:} There is obvious distribution imbalance in tensorflow. Taking inception as a example, most data is located on package 0. And the Latency is seriously affected by the Imbalance. The Memory Latency and Memory Accessing Imbalance of inception is shown in Table \ref{tab:LatencyAndImbalance}. Almost all operations have a high imbalance which leads to great fluctuation of memory access latency. 

\textbf{Observation 2:} The result of Remote Access Ratio is shown in figure xxx. It is high in all tests, which means the data-locality problem it is limiting the performance of tensorflow. 

This comes from the thread and memory managements of tensorflow. The threads management module of tensorflow is built on the threadpool of eigen library, which does not provide a NUMA awareness interface. There are two thread pools, one for the inter-parallel (inter-pool), and the other one for intra-parallel (intra-pool). The management of memory location obey the first touch policy, and the location of threads obey the xxx policy. Every time tensorflow executes a new operation, it gets a thread from inter-pool. This thread will initialize the operation, which include get the data from input(s) and malloc space form output(s). Generally, the input data comes from operation(s) the new operation depends on. And because of the first touch policy, the input(s) is located at the local memory of depended operation(s), and the outputs will be put on the local memory of the inter-thread. Then, the inter-thread will bring up intra-thread(s) to run the new operation. The xxx policy of thread location provides no guarantee if these new intra-threads will be in the same processor as the inter-thread or not.

So, there are two problems to solve to achieve best performance of NUMA architecture: (1) equably distributing data for different operations separately to different DRAMs; (2) run the operations on processors which hold the data locally. We have a detail description of our memory management model in chapter xxx and the realization in chapter xxx.\\




\begin{comment}
\textbf{Observation 1.} Each training step includes a few large operations and many small operations; ---> runtime design: 

\textbf{Observation 2.} At any moment, there are at most 3 operations ready to launch.  %--> runtime design: inter-op parallelism

\textbf{Observation 3.} The time accumulation of small operations is big; 
%-> runtime design: we cannot ignore small operations.
\end{comment}





